Double Dimer Covers on Snake Graphs from Super Cluster Expansions

In a recent paper, the authors gave combinatorial formulas for the Laurent expansions of super $\lambda$-lengths in a marked disk, generalizing Schiffler's $T$-path formula. In the present paper, we give an alternate combinatorial expression for these super $\lambda$-lengths in terms of double dimer covers on snake graphs. This generalizes the dimer formulas of Musiker, Schiffler, and Williams.

==> figures/snake-graph-d.tex <==
\begin {tikzpicture}[scale=1]
    \draw (0,0) -- (-1,0) -- (-1,1) -- (0,1);
    \draw (0,0) -- ++(2,0) -- ++(0,1) -- ++(1,0) -- ++(0,2) -- ++(-1,0) -- ++(0,-1) -- ++(-1,0) -- ++(0,-1) -- ++(-1,0) -- cycle;
    \draw (1,0) -- ++(0,1) -- ++(1,0) -- ++(0,1) -- ++(1,0);
    \draw (3,2) -- ++(1,0) -- ++(0,1) -- ++(-1,0);

    \draw (-1.5,0.5) node {$\cdots$};

    \draw (2.5,3) node[above] {$e_1$};

    \draw (3.5,3) node[above] {$b$};
    \draw[blue, line width = 2] (3,3) -- (4,3);

    \draw (3.5,2) node[below] {$e_2$};
    \draw (3,1.5) node[right] {$e_2$};
    \draw[blue, line width = 2] (3,2) -- (4,2);

    \draw (1.5,2) node[above] {$e_3$};
    \draw (2,2.5) node[left]  {$e_3$};
    \draw[blue, line width = 2] (2,2) -- (2,3);

    \draw (2.5,1) node[below] {$e_4$};
    \draw (2,0.5) node[right] {$e_4$};
    \draw[blue, line width = 2] (2,1) -- (3,1);

    \draw (1,1.5) node[left]  {$e_5$};
    \draw (0.5,1) node[above] {$e_5$};
    \draw[blue, line width = 2] (1,1) -- (1,2);

    \draw (1.5,0) node[below] {$e_6$};
    \draw[blue, line width = 2] (1,0) -- (2,0);
\end {tikzpicture}
\quad
\begin {tikzpicture}[scale=1]
    
    \draw [dashed] (0,0) -- ++(2,0) -- ++(0,1) -- ++(1,0) -- ++(0,2) -- ++(-1,0) -- ++(0,-1) -- ++(-1,0) -- ++(0,-1) -- ++(-1,0) ;
    \draw (0,0) -- (-1,0) -- (-1,1) -- (0,1)--cycle;
    \draw[dashed] (1,0) -- ++(0,1) -- ++(1,0) -- ++(0,1) -- ++(1,0);
    \draw[dashed] (3,2) -- ++(1,0) -- ++(0,1) -- ++(-1,0);
    \draw (1.5,0) node[below] {$\color{white}e_6$};

    \draw (-1.5,0.5) node {$\cdots$};

 
\end {tikzpicture}
